Rethinking Mesh Watermark: Towards Highly Robust and Adaptable Deep 3D Mesh Watermarking

The goal of 3D mesh watermarking is to embed the message in 3D meshes that can withstand various attacks imperceptibly and reconstruct the message accurately from watermarked meshes. The watermarking algorithm is supposed to withstand multiple attacks, and the complexity should not grow significantly with the mesh size. Unfortunately, previous methods are less robust against attacks and lack of adaptability. In this paper, we propose a robust and adaptable deep 3D mesh watermarking Deep3DMark that leverages attention-based convolutions in watermarking tasks to embed binary messages in vertex distributions without texture assistance. Furthermore, our Deep3DMark exploits the property that simplified meshes inherit similar relations from the original ones, where the relation is the offset vector directed from one vertex to its neighbor. By doing so, our method can be trained on simplified meshes but remains effective on large size meshes (size adaptable) and unseen categories of meshes (geometry adaptable). Extensive experiments demonstrate our method remains efficient and effective even if the mesh size is 190x increased. Under mesh attacks, Deep3DMark achieves 10%~50% higher accuracy than traditional methods, and 2x higher SNR and 8% higher accuracy than previous DNN-based methods.

==> chapter/method1.tex <==


\section{Definition} \label{sec: def}
%TODO prove your method is permutation invariant, rotation invariant
Triangle mesh can be represented as $\mathcal{M}(V,F)$. Vertices $V\in \mathbb{R}^{N_v\times C_v}$ contains $N_v$ vertices, and each vertex has $C_v$ vertex elements such as coordinates and normals. Faces $F\in \{0, ..., N_v-1\}^{N_f\times 3}$ contains $N_f$ faces, each of which contains vertex indices. Since changes of faces $F$ will produce unexpected artifacts, we embed a binary message $M\in\{0,1\}^{N_m}$ into the vertex distribution $V$, i.e., we encode the secret message by bringing distortions into $V$. Let $V,\hat{V},M,\hat{M}$ denote the origin vertex, watermarked vertex, binary messages, and reconstructed messages, respectively. We model the problem by the following equation:
\begin{equation}
    \label{eq:problem}
    \begin{gathered}
        \hat{V} = \mathcal{E}_\phi(V, M)\\
        \hat{M} = \mathcal{D}_\theta(\hat{V})
    \end{gathered}
\end{equation}
In Eq \ref{eq:problem}, a parameterized encoding function $\mathcal{E}_\phi$ generates watermarked vertices $\hat{V}$ given original vertices $V$ and a binary message $M$. A parameterized decoding function $\mathcal{D}_\theta$ reconstructs $\hat{M}$ from $\hat{V}$. The encoding function should minimize the perturbation between $V$ and $\hat{V}$ by minimizing the following loss to achieve imperceptible embedding:
\begin{equation}
    \label{eq:obj1}
    \begin{aligned}
        &L_{enc}(\phi, \theta)=\mathbb{E}_{V,M}[\lVert \hat{V} - V \rVert_2^2]
    \end{aligned}
\end{equation}
To achieve precise reconstruction, we try to minimize the following loss:
\begin{equation}
    \label{eq:obj2}
    \begin{aligned}
        &L_{dec}(\phi, \theta)=\mathbb{E}_{V,M}[\lVert \hat{M} - M \rVert_2^2]
    \end{aligned}
\end{equation}
Finally, we have combined the optimization problem:
\begin{equation}
    \label{eq:finalobj}
    \phi^{*}, \theta^{*} = \argmin_{\phi, \theta} (L_{enc}(\phi, \theta) + L_{dec}(\phi, \theta))
\end{equation}

\section{Consistent Neighborhood Convolution}\label{sec:cnc}
Consistent Neighborhood convolution (CNC) is a convolution operator designed for robust and imperceptible watermarking. We design it by exploiting the similarity between image watermarking and 3D object watermarking. Section \ref{sec:background} introduces the way of image watermarking and lists several simple but vital properties in image watermarking tasks. We propose our CNC in Section \ref{sec:ourapproach}, which serves as the backbone of our WM-GAN.
\subsection{Background} \label{sec:background}

2D image $\mathbf{F}(x,y)$ can be viewed as a weighted graph signal where points are indexed by discrete 2D grid offset $(x,y)\in \mathbb{N}^2$, edges connect adjacent points and weights are the RGB values of points. Traditional CNN is to apply a filter matrix $\mathbf{W}$ of size $(2m+1,2n+1)$ to an image. In this case, the point $(x,y)$ is adjacent to points $(x+\delta x, y+\delta y)$, where $\delta x\in \{-m,...,-1,0,1,...,m\}$, and $\delta y\in\{-n,...,-1,0,1,...,n\}$. Then we can view traditional CNN in a graph way (Eq.(\ref{eq:grapical_cnn})).
\begin{equation}
    \begin{aligned}
        \mathbf{F}(x,y) = \sum_{(\delta x, \delta y) \in \mathcal{N}(x,y)}\mathbf{W}(\delta x,\delta y)\mathbf{F}(x-\delta x,y-\delta y)
    \end{aligned}
    \label{eq:grapical_cnn}
\end{equation}
where $\mathcal{N}(x,y)$ is the set of points adjacent $(x,y)$, and the filter matrix $W$ can be viewed as a function mapping from grid offsets $(\delta x, \delta y)$ to filter weights.

Based on the understanding above, we dive into the image watermarking task in \cite{zhu2018hidden}, which uses stacked CNNs to model both $\mathcal{E}_{\phi}$ and $\mathcal{D}_{\theta}$ (Fig. \ref{fig:img_wm}). Here we list several vital properties that significantly impact the quality of watermarking.
\begin{itemize}
    \item Property 1. Grid offsets $(\delta x, \delta y)$ are defined on discrete 2D space, and thus the filter matrix $W$ is optimized on the finite set of grid offsets.
    \item Property 2. Grid offsets $(\delta x, \delta y)$ are independent of the convolution results of the previous layer, and thus the filter matrix $W$ is optimized on the fixed set of grid offsets.
    \item Property 3. Topology is independent of convolution results of the previous layer, and thus filter matrices $W$ of both $\mathcal{E}_{\phi}$ and $\mathcal{D}_{\theta}$ are optimized on the consistent topology. Because the relative relation between pixels is always fixed.
\end{itemize}
In the next subsection, we statistically show that these properties are not easy to satisfy due to the irregular nature of the 3D object.

\begin{figure}
    \centering
    % \begin{subfigure}[b]{\linewidth}
    %     \includegraphics[width=\linewidth]{figures/method/img_wm.png}
    %     \caption{L1 Norm Difference}
    % \end{subfigure}
    % \\
    % \begin{subfigure}[b]{\linewidth}
    %     \includegraphics[width=\linewidth]{figures/method/mesh_wm.png}
    %     \caption{Original}
    % \end{subfigure}
    \includegraphics[width=\linewidth]{figures/method/img_wm.png}
    \caption{Image watermarking process using CNN.}
    \label{fig:img_wm}
\end{figure}

\subsection{Our Approach} \label{sec:ourapproach}

3D mesh $\mathcal{M}(V,F)$ can be viewed as a weighted graph signal where points are located by continuous 3D index $(x,y,z)$, edge information is maintained by the face set $F$ and the weights are features $\mathbf{F}$ of points. We follow the convention in \cite{simonovsky2017ecc, wu2019pointconv, liu2019rscnn} and define the offset between the point $\mathbf{v_i}=(x_i,y_i,z_i)$ and the point $\mathbf{v_j}=(x_j,y_j,z_j)$ as $\mathbf{D}(\mathbf{v_i}, \mathbf{v_j})=\mathbf{v_i}-\mathbf{v_j}$. We define convolution on 3D mesh as
\begin{equation}
    \begin{gathered}
        \mathbf{F}^{l+1}(\mathbf{v_i})=\frac{1}{|\mathcal{N}(\mathbf{v_i})|}\sum_{\mathbf{v_j}\in \mathcal{N}(\mathbf{v_i})}\mathbf{F}^l(\mathbf{v_j})\mathbf{W}(\mathbf{D}(\mathbf{v_j},\mathbf{v_i}))\\
        \mathbf{W}(\mathbf{d}) = MLP(\mathbf{d})\\
    \end{gathered}
    \label{eq:3Dconv}
\end{equation}
where $\mathbf{F}^l$ are the feature vector of output from layer $l$.

%TODO statistic prove consistent topology & ECC fail

\textbf{Challenges and Solution.} We show that it is not easy to fit all Properties listed in the last subsection. Since points $f(x,y,z)$ are defined on continuous 3D space, traditional CNN cannot be applied to 3D point convolution (violates Property 1). We adopt an MLP to learn the filter matrix Besides, watermarking in 3D points (Eq.(\ref{eq:problem})) brings distortions to the original point set $V$ to generate watermarked point set $\hat{V}$, which makes point offset dependent on the result of convolution (violates Property 2). We can incorporate original mesh topology to construct neighbors $\mathcal{N}(\mathbf{v})$, but edges of meshes can connect points far from each other (Property 4). Another approach to construct neighbors $\mathcal{N}(\mathbf{v})$ is to perform k neighbor query over for each $\mathbf{v}$ and pass 




\subsection{Comparison to Existing Methods}


\section{Generation-based 3D Watermarking}

Our goal is to train an end-to-end generation network for imperceptible mesh watermarking that can be robust to arbitrary attacks. We first introduce general problem definition and objectives in Sec. \ref{sec: def}. Then we introduce our architecture and workflow in Sec. \ref{sec: arch}, followed by a detailed introduction of our improved convolution operator in Sec. \ref{sec: cnc}, which is commonly used in our architecture. Sec. \ref{sec: loss} introduce details of our training.

% Triangle mesh $\mathcal{M}(V,F)$ can be viewed as the joint distribution of two independent variables $V$ and $F$. Vertices $V\in \mathbb{R}^{N_v\times C_v}$ contains $N_v$ vertices and each vertices have $C_v$ vertex elements such as coordinates and normals. Faces $F\in \{0, ..., N_v-1\}^{N_f\times 3}$ contains $N_f$ faces, each of which contains vertex indices. We embed a binary message $M\in\{0,1\}^{N_m}$ into the vertex distribution $V$ because the change of faces $F$ will produce unexpected artifacts \cite{yoo2022deep}. Let $V,\hat{V},M,\hat{M}$ denote random variables of origin vertex, watermarked vertex, binary messages and reconstructed messages respectively. We model their joint distribution using the following graphic model:
% \begin{equation}
%     \label{eq: 1}
%     \begin{aligned}
%     &p(v,m,\hat{v},\hat{m})=\\
%     &p_{\text{vertex}}(v)p_{\text{message}}(m)p_{\text{enc}}(\hat{v}|v,m;\phi)p_{\text{dec}}(\hat{m}|\hat{v};\theta)
%     \end{aligned}
% \end{equation}
% In Eq \ref{eq: 1}, $p_{\text{vertex}}(v)$ and $p_{\text{message}}$ are distributions of vertices and binary messages respectively and can be accessible through samples. A learnable encoder $p_{\text{enc}}(\hat{v}|v,m;\phi)$ generates watermarked vertices $\hat{v}$ given $v$ and $m$. A learnable decoder $p_{\text{dec}}(\hat{m}|\hat{v};\theta)$ reconstructs $\hat{m}$ from $\hat{v}$. To achieve imperceptible embedding, the perturbation between $v$ and $\hat{v}$ should be minimized, and thus we minimize the following loss:
% \begin{equation}
%     \label{eq: 2}
%     \begin{aligned}
%         &L_{enc}(\phi, \theta)=\\
%         &\mathbb{E}_{m\sim p_{\text{message}}(m)}\mathbb{E}_{v\sim p_{\text{vertex}}(v)}\mathbb{E}_{\hat{v}\sim p_{\text{enc}}(\hat{v}|v,m;\phi)}[\hat{v}-v]
%     \end{aligned}
% \end{equation}
% To achieve precise reconstruction, we try to minimize the following loss:
% \begin{equation}
%     \begin{aligned}
%         &L_{dec}(\phi, \theta)=\\
%         &\mathbb{E}_{m\sim p_{\text{message}}(m)}\mathbb{E}_{v\sim p_{\text{vertex}}(v)}\mathbb{E}_{\hat{v}\sim p_{\text{enc}}(\hat{v}|v,m;\phi)}[-logp_{\text{dec}}(m|\hat{v})]
%     \end{aligned}
% \end{equation}
% Finally, we have combined optimization problem:
% \begin{equation}
%     \phi^{*}, \theta^{*} = \argmin_{\phi, \theta} (L_{enc}(\phi, \theta) + L_{dec}(\phi, \theta))
% \end{equation}

\subsection{Network Architecture} \label{sec: arch}
We deploy a GAN-based network (Figure \ref{fig:arch}) to achieve objectives in Eq. \ref{eq:finalobj}. Our architecture consists of five components: 1) a message autoencoder map a binary message $M$ to a latent code $z$ and decoder $z$ back to $M$, 2) a learnable encoder $\mathbf{E}$ simulate function $\mathcal{E}$ that generate a watermarked vertices $\hat{V}$ given $V$ and $z$, 3) an attack layer apply perturbation over $\hat{V}$ to increase the robustness in the way of data augmentation, 4) a decoder $\mathbf{D}$ simulate $\mathcal{D}$ that reconstruct binary message from $\hat{v}$, and 5) a discriminator $\mathbf{A}$ encourage $\hat{V}$ indistinguishable from $V$. Since CNN has been proven to be successful in image watermarking \cite{zhu2018hidden}, it is natural for us to use a 3D convolution operator such as PointConv \cite{wu2019pointconv} and RSCNN \cite{liu2019rscnn} in our watermarking task. However, our attempts to incorporate PointConv or RSCNN to achieve a robust and imperceptible watermark have been unsuccessful. Hence, we design Consistent Neighbor Convolution (CNC) (Sec. \ref{sec: cnc}), which serves as the backbone of our $\mathbf{E}$, $\mathbf{D}$, and $\mathbf{A}$.

The \textbf{encoder} $\mathbf{E}$ first applies CNC convolutions to input $V$ to form some intermediate representation. We aim to incorporate message latent code $z$ in the way that the encoder learns to embed parts of it at any spatial location of $V$. To achieve this, we replicate the latent code and concatenate it to the intermediate representations. We apply more CNC convolutions to transform the concatenated feature to watermarked vertices $\hat{V}$. 
The \textbf{attack layer} applies perturbations over generated $\hat{V}$. We apply several mesh attacks, including 1) cropping attack with cropping ratio $c$, 2) Gaussian noise with mean $\mu$ and deviation $\sigma$, 3) rotation attack along the center with parameters $(\alpha, x, y, z)$, 4) translation attack, and 5) scaling attack with a parameter $s$.
The \textbf{decoder} $\mathbf{D}$ first applies several CNC convolutions to generate the intermediate representation of $\hat{V}$. It finally applies a global average pooling followed by an MLP layer to generate a vector of the same size as the latent code $z$. The average pooling layer ensures that the decoder aggregates information from all vertices. The \textbf{adversarial discriminator} $\mathbf{A}$ shares a similar structure as the decoder except that its final MLP layer transforms the aggregated vector into a binary classification, which means whether or not the given $\hat{V}$ is generated by the encoder $\mathbf{E}$.

According to Shannon's capacity theory, redundancy is necessary to achieve robustness. The \textbf{message autoencoder} increases the robustness of our system by injecting redundancy into the system. Given a binary message $M$ of length $N_m$, the message encoder encodes it into a latent code $z$ of length $N_z>N_m$, which can be used to recover $M$ through a message decoder. We train the autoencoder in a way that the decoder can recover $M$ from the noised latent code $\hat{z}$. We choose NECST \cite{choi2019necst}, a learnable channel coding method, as our message autoencoder. Note that the message autoencoder is trained independently from the entire watermarking model.




\subsection{Training and Losses} \label{sec: loss}
\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz_diff.png}
        \caption{L1 Norm Difference}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz.png}
        \caption{Original}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz_enc.png}
        \caption{Watermarked}
    \end{subfigure}
    \caption{Example meshes: (a) visualization of L1 Norm distortions per vertex normal, (b) original meshes and (c) watermarked meshes with CNC (ours) being used in architecture}
    \label{fig: mesh_quality}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz.png}
        \caption{Cover Mesh $\mathcal{M}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_enc.png}
        \caption{Stego Mesh $\hat{\mathcal{M}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_0.png}
        \caption{Gauss Noise($\mu=0.1$, $\sigma=0.001$)}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_1.png}
        \caption{Rotation}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_2.png}
        \caption{Scaling $s=0.7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_3.png}
        \caption{Cropping Attack $c=50\%$}
    \end{subfigure}
    \caption{Example mesh under different attack.}
    \label{fig: mesh_quality}
\end{figure*}

We achieve the objective in Eq \ref{eq:finalobj} using three losses: encoding loss $L_{enc}$, reconstruction loss $L_{dec}$, and discriminative loss $L_{dis}$. Formally:
\begin{equation}
    \begin{aligned}
        &\phi^*, \theta^*=\\
        &\argmin_{\phi, \theta}(\lambda_{enc} L_{enc}(\phi, \theta) + \lambda_{dec} L_{dec}(\phi, \theta) + \lambda_{dis} L_{dis}(\phi, \theta))
    \end{aligned}
\end{equation}
where $\lambda_{enc},\lambda_{dec},\lambda_{dis}$ are weight factors. Both $L_{enc}, L_{dis}$ encourage generated $\hat{V}$ indistinguishable from $V$. For $L_{enc}$, we use both L2 norm and infinite norm of geometry difference to penalize the distortion:
\begin{equation}
    L_{enc}=\frac{1}{N_v}\sum_{i}^{N_v}(V[i] - \hat{V}[i])^2 + \max_i\{V[i]-\hat{V}[i]\}
\end{equation}
For $L_{dis}$, we use part of sigmoid cross entropy loss:
\begin{equation}
    L_{dis}=\log(1-\sigma(\mathbf{A}(\hat{V})))
\end{equation}
We apply standard sigmoid cross entropy loss to encourage precise message reconstruction:
\begin{equation}
    \begin{aligned}
        &L_{dec}=\\
        &\frac{1}{N_m}\sum_{i}^{N_m}(M[i]\cdot\log\sigma(\hat{M}[i]) + (1-M[i])\cdot\log\sigma(1-\hat{M}[i]))
    \end{aligned}
\end{equation}


The final message bits get from by clipping:
\begin{equation}
    M_{final}=clip(sign(\hat{M}-0.5), 0, 1)
\end{equation}

%TODO figure interpret pointconv convolution

%TODO sampling (evidence)
%TODO nearest grouping (evidence)
%TODO consistent topology selection (evidence)

==> chapter/method2.tex <==


\section{Method}

Our goal is to train an end-to-end generation network for imperceptible mesh watermarking that can be robust to arbitrary attacks. We first introduce general problem definition and objectives in Sec. \ref{sec: def}. Then we introduce our architecture and workflow in Sec. \ref{sec: arch}, followed by a detailed introduction of our improved convolution operator in Sec. \ref{sec: cnc}, which is commonly used in our architecture. Sec. \ref{sec: loss} introduce details of our training.

\subsection{Definition} \label{sec: def}
%TODO prove your method is permutation invariant, rotation invariant
Triangle mesh can be represented as $\mathcal{M}(V,F)$. Vertices $V\in \mathbb{R}^{N_v\times C_v}$ contains $N_v$ vertices, and each vertex has $C_v$ vertex elements such as coordinates and normals. Faces $F\in \{0, ..., N_v-1\}^{N_f\times 3}$ contains $N_f$ faces, each of which contains vertex indices. We embed a binary message $M\in\{0,1\}^{N_m}$ into the vertex distribution $V$ because the change of faces $F$ will produce unexpected artifacts \cite{yoo2022deep}. Let $V,\hat{V},M,\hat{M}$ denote the origin vertex, watermarked vertex, binary messages, and reconstructed messages, respectively. We model the problem by the following equation:
\begin{equation}
    \label{eq:problem}
    \begin{gathered}
        \hat{V} = \mathcal{E}_\phi(V, M)\\
        \hat{M} = \mathcal{D}_\theta(\hat{V})
    \end{gathered}
\end{equation}
In Eq \ref{eq:problem}, a parameterized encoding function $\mathcal{E}_\phi$ generates watermarked vertices $\hat{V}$ given original vertices $V$ and a binary message $M$. A parameterized decoding function $\mathcal{D}_\theta$ reconstructs $\hat{M}$ from $\hat{V}$. The encoding function should minimize the perturbation between $V$ and $\hat{V}$ by minimizing the following loss to achieve imperceptible embedding:
\begin{equation}
    \label{eq:obj1}
    \begin{aligned}
        &L_{enc}(\phi, \theta)=\mathbb{E}_{V,M}[\lVert \hat{V} - V \rVert_2^2]
    \end{aligned}
\end{equation}
To achieve precise reconstruction, we try to minimize the following loss:
\begin{equation}
    \label{eq:obj2}
    \begin{aligned}
        &L_{dec}(\phi, \theta)=\mathbb{E}_{V,M}[\lVert \hat{M} - M \rVert_2^2]
    \end{aligned}
\end{equation}
Finally, we have combined the optimization problem:
\begin{equation}
    \label{eq:finalobj}
    \phi^{*}, \theta^{*} = \argmin_{\phi, \theta} (L_{enc}(\phi, \theta) + L_{dec}(\phi, \theta))
\end{equation}

% Triangle mesh $\mathcal{M}(V,F)$ can be viewed as the joint distribution of two independent variables $V$ and $F$. Vertices $V\in \mathbb{R}^{N_v\times C_v}$ contains $N_v$ vertices and each vertices have $C_v$ vertex elements such as coordinates and normals. Faces $F\in \{0, ..., N_v-1\}^{N_f\times 3}$ contains $N_f$ faces, each of which contains vertex indices. We embed a binary message $M\in\{0,1\}^{N_m}$ into the vertex distribution $V$ because the change of faces $F$ will produce unexpected artifacts \cite{yoo2022deep}. Let $V,\hat{V},M,\hat{M}$ denote random variables of origin vertex, watermarked vertex, binary messages and reconstructed messages respectively. We model their joint distribution using the following graphic model:
% \begin{equation}
%     \label{eq: 1}
%     \begin{aligned}
%     &p(v,m,\hat{v},\hat{m})=\\
%     &p_{\text{vertex}}(v)p_{\text{message}}(m)p_{\text{enc}}(\hat{v}|v,m;\phi)p_{\text{dec}}(\hat{m}|\hat{v};\theta)
%     \end{aligned}
% \end{equation}
% In Eq \ref{eq: 1}, $p_{\text{vertex}}(v)$ and $p_{\text{message}}$ are distributions of vertices and binary messages respectively and can be accessible through samples. A learnable encoder $p_{\text{enc}}(\hat{v}|v,m;\phi)$ generates watermarked vertices $\hat{v}$ given $v$ and $m$. A learnable decoder $p_{\text{dec}}(\hat{m}|\hat{v};\theta)$ reconstructs $\hat{m}$ from $\hat{v}$. To achieve imperceptible embedding, the perturbation between $v$ and $\hat{v}$ should be minimized, and thus we minimize the following loss:
% \begin{equation}
%     \label{eq: 2}
%     \begin{aligned}
%         &L_{enc}(\phi, \theta)=\\
%         &\mathbb{E}_{m\sim p_{\text{message}}(m)}\mathbb{E}_{v\sim p_{\text{vertex}}(v)}\mathbb{E}_{\hat{v}\sim p_{\text{enc}}(\hat{v}|v,m;\phi)}[\hat{v}-v]
%     \end{aligned}
% \end{equation}
% To achieve precise reconstruction, we try to minimize the following loss:
% \begin{equation}
%     \begin{aligned}
%         &L_{dec}(\phi, \theta)=\\
%         &\mathbb{E}_{m\sim p_{\text{message}}(m)}\mathbb{E}_{v\sim p_{\text{vertex}}(v)}\mathbb{E}_{\hat{v}\sim p_{\text{enc}}(\hat{v}|v,m;\phi)}[-logp_{\text{dec}}(m|\hat{v})]
%     \end{aligned}
% \end{equation}
% Finally, we have combined optimization problem:
% \begin{equation}
%     \phi^{*}, \theta^{*} = \argmin_{\phi, \theta} (L_{enc}(\phi, \theta) + L_{dec}(\phi, \theta))
% \end{equation}

\subsection{Network Architecture} \label{sec: arch}
We deploy a GAN-based network (Figure \ref{fig:arch}) to achieve objectives in Eq. \ref{eq:finalobj}. Our architecture consists of five components: 1) a message autoencoder map a binary message $M$ to a latent code $z$ and decoder $z$ back to $M$, 2) a learnable encoder $\mathbf{E}$ simulate function $\mathcal{E}$ that generate a watermarked vertices $\hat{V}$ given $V$ and $z$, 3) an attack layer apply perturbation over $\hat{V}$ to increase the robustness in the way of data augmentation, 4) a decoder $\mathbf{D}$ simulate $\mathcal{D}$ that reconstruct binary message from $\hat{v}$, and 5) a discriminator $\mathbf{A}$ encourage $\hat{V}$ indistinguishable from $V$. Since CNN has been proven to be successful in image watermarking \cite{zhu2018hidden}, it is natural for us to use a 3D convolution operator such as PointConv \cite{wu2019pointconv} and RSCNN \cite{liu2019rscnn} in our watermarking task. However, our attempts to incorporate PointConv or RSCNN to achieve a robust and imperceptible watermark have been unsuccessful. Hence, we design Consistent Neighbor Convolution (CNC) (Sec. \ref{sec: cnc}), which serves as the backbone of our $\mathbf{E}$, $\mathbf{D}$, and $\mathbf{A}$.

The \textbf{encoder} $\mathbf{E}$ first applies CNC convolutions to input $V$ to form some intermediate representation. We aim to incorporate message latent code $z$ in the way that the encoder learns to embed parts of it at any spatial location of $V$. To achieve this, we replicate the latent code and concatenate it to the intermediate representations. We apply more CNC convolutions to transform the concatenated feature to watermarked vertices $\hat{V}$. 
The \textbf{attack layer} applies perturbations over generated $\hat{V}$. We apply several mesh attacks, including 1) cropping attack with cropping ratio $c$, 2) Gaussian noise with mean $\mu$ and deviation $\sigma$, 3) rotation attack along the center with parameters $(\alpha, x, y, z)$, 4) translation attack, and 5) scaling attack with a parameter $s$.
The \textbf{decoder} $\mathbf{D}$ first applies several CNC convolutions to generate the intermediate representation of $\hat{V}$. It finally applies a global average pooling followed by an MLP layer to generate a vector of the same size as the latent code $z$. The average pooling layer ensures that the decoder aggregates information from all vertices. The \textbf{adversarial discriminator} $\mathbf{A}$ shares a similar structure as the decoder except that its final MLP layer transforms the aggregated vector into a binary classification, which means whether or not the given $\hat{V}$ is generated by the encoder $\mathbf{E}$.

According to Shannon's capacity theory, redundancy is necessary to achieve robustness. The \textbf{message autoencoder} increases the robustness of our system by injecting redundancy into the system. Given a binary message $M$ of length $N_m$, the message encoder encodes it into a latent code $z$ of length $N_z>N_m$, which can be used to recover $M$ through a message decoder. We train the autoencoder in a way that the decoder can recover $M$ from the noised latent code $\hat{z}$. We choose NECST \cite{choi2019necst}, a learnable channel coding method, as our message autoencoder. Note that the message autoencoder is trained independently from the entire watermarking model.

\subsection{Consistent Neighbor Convolution} \label{sec: cnc}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/method/conv_diff.pdf}
    \caption{Image grad vs. 3D vertices. (a) and (b) shows local regions centered at $v_i$ in the case of image and 3D vertices, respectively. $R(v_j, v_i)$ in (a) denotes the grid offset $(\mathrm{d}x, \mathrm{d}y)=(-1, 0)$, while in (b) denotes euclidean distance $\mathrm{d}v$. (c) shows the case when $v_i$ shifts to $v_i'$, resulting in non-deterministic neighborhood selection. (d) shows an extreme case of non-uniform neighbor selection.}
    \label{fig:conv_diff}
\end{figure}

%TODO: figure prove sampling effect when applying watermark
In this section, we propose Consistent Neighbor Convolution (CNC), which is the backbone of our entire architecture. We develop CNC based on two insights: 1) consistent and deterministic neighbors selection between convolution layers can achieve significant improvements in 3D watermarking, and 2) strategies of sampling and neighbor selection significantly impact the effectiveness of watermarking.

\textbf{Convolution definition.} We start from the continuous version of convolution:
\begin{equation*}
    \begin{aligned}
        &\text{In 2D}\quad \mathbf{F}(x,y)=\\
        &\iint\displaylimits_{\delta x\,\delta y} \mathbf{F}(x+\delta x,y+\delta y)\mathbf{W}(\delta x,\delta y) \,d\delta x\,d\delta y\\
        &\text{In 3D}\quad \mathbf{F}(x,y,z)=\\
        &\iiint\displaylimits_{\delta x\,\delta y\,\delta z} \mathbf{F}(x+\delta x,y+\delta y,z+\delta z)\mathbf{W}(\delta x,\delta y,\delta z) \,d\delta x\,d\delta y\,d\delta z\\
    \end{aligned}
\end{equation*}
where $\mathbf{F}$ is the feature vector and $\mathbf{W}$ is the filter matrix applied over feature vectors of each local region. We can easily transform this formula into a more generalized and discretized version:
\begin{equation}
    \mathbf{F}(v_i)=\sum_{v_j\in \mathcal{N}(v_i)}\mathbf{F}(v_j)\mathbf{W}(R(v_j,v_i))
\end{equation}
where $\mathcal{N}(v_i)$ denotes the local region around $v_i$ and function $R$ gives the relationship between $v_i$ and $v_j$. In classic CNN, $v_i$ can be a channel vector of a single pixel, and $R(v_i, v_j)$ can denote the grid offset $(\mathrm{d}x, \mathrm{d}y)\in \mathbb{N}^2$ between pixels $v_i$ and $v_j$. In 3D point convolution, $v_i$ can be an element vector of a single point, $R(v_i, v_j)$ can denote their euclidean distance $\mathrm{d}v\in R$. 

\textbf{Challenges.} Figure \ref{fig:conv_diff} lists several major challenges when constructing 3D point convolution for watermarking tasks. The first challenge is that $R(v_i, v_j)$ in 3D vertices distribute in continuous space, and thus discretized convolution filters are not applicable. The second challenge is that the change of 3D vertex elements such as vertex coordinates affects both $\mathcal{N}(v_i)$ and $R(v_j, v_i)$. As is shown in Figure \ref{fig:conv_diff} (c), in generation tasks, $v_i$ can be shifted to the place of $v_1'$ after several batches of optimization. This causes non-deterministic and inconsistent neighbor selection and makes optimization hard to converge. The third challenge is that 3D vertices are non-uniformly sampled, which results in non-uniform neighbor selection. In the extreme case, as is shown in Figure \ref{fig:conv_diff} (d), $v_i$ and $v_j$ select the same set of neighbors, while the rest of the vertices are ignored. We solve these challenges one by one. To acquire filter matrix $\mathbf{W}$ over continuous space, we deploy an MLP to generate filter matrix $W$ when given $R(v_i,v_j)$. To ensure deterministic and uniform neighbor selection, we intuitively incorporate face information into the neighbor selection process and apply graph convolution. However, such attempts do not perform well in watermark tasks. One reason is that neighbor selection based on graph information is also non-uniform. Another is that faces in mesh usually connect vertices that distribute far from each other, which makes DNN hard to learn their relations. Our final solution is to apply the K neighbor query for each vertex of $V$ and transfer $\mathcal{N}(v)$ across all layers of convolutions. 


\subsection{Training and Losses} \label{sec: loss}
\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz_diff.png}
        \caption{L1 Norm Difference}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz.png}
        \caption{Original}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/xyz_enc.png}
        \caption{Watermarked}
    \end{subfigure}
    \caption{Example meshes: (a) visualization of L1 Norm distortions per vertex normal, (b) original meshes and (c) watermarked meshes with CNC (ours) being used in architecture}
    \label{fig: mesh_quality}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz.png}
        \caption{Cover Mesh $\mathcal{M}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_enc.png}
        \caption{Stego Mesh $\hat{\mathcal{M}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_0.png}
        \caption{Gauss Noise($\mu=0.1$, $\sigma=0.001$)}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_1.png}
        \caption{Rotation}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_2.png}
        \caption{Scaling $s=0.7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\linewidth}
        \includegraphics[width=\linewidth]{figures/experiments/robustness/xyz_noise_3.png}
        \caption{Cropping Attack $c=50\%$}
    \end{subfigure}
    \caption{Example mesh under different attack.}
    \label{fig: mesh_quality}
\end{figure*}

We achieve the objective in Eq \ref{eq:finalobj} using three losses: encoding loss $L_{enc}$, reconstruction loss $L_{dec}$, and discriminative loss $L_{dis}$. Formally:
\begin{equation}
    \begin{aligned}
        &\phi^*, \theta^*=\\
        &\argmin_{\phi, \theta}(\lambda_{enc} L_{enc}(\phi, \theta) + \lambda_{dec} L_{dec}(\phi, \theta) + \lambda_{dis} L_{dis}(\phi, \theta))
    \end{aligned}
\end{equation}
where $\lambda_{enc},\lambda_{dec},\lambda_{dis}$ are weight factors. Both $L_{enc}, L_{dis}$ encourage generated $\hat{V}$ indistinguishable from $V$. For $L_{enc}$, we use both L2 norm and infinite norm of geometry difference to penalize the distortion:
\begin{equation}
    L_{enc}=\frac{1}{N_v}\sum_{i}^{N_v}(V[i] - \hat{V}[i])^2 + \max_i\{V[i]-\hat{V}[i]\}
\end{equation}
For $L_{dis}$, we use part of sigmoid cross entropy loss:
\begin{equation}
    L_{dis}=\log(1-\sigma(\mathbf{A}(\hat{V})))
\end{equation}
We apply standard sigmoid cross entropy loss to encourage precise message reconstruction:
\begin{equation}
    \begin{aligned}
        &L_{dec}=\\
        &\frac{1}{N_m}\sum_{i}^{N_m}(M[i]\cdot\log\sigma(\hat{M}[i]) + (1-M[i])\cdot\log\sigma(1-\hat{M}[i]))
    \end{aligned}
\end{equation}


The final message bits get from by clipping:
\begin{equation}
    M_{final}=clip(sign(\hat{M}-0.5), 0, 1)
\end{equation}

%TODO figure interpret pointconv convolution

%TODO sampling (evidence)
%TODO nearest grouping (evidence)
%TODO consistent topology selection (evidence)

==> chapter/method4.tex <==
\section{Bridge the gap Between Image Watermarking and Mesh Watermarking}\label{sec:bridge}
In this section, we design the convolution for mesh watermarking by exploiting the similarity between mesh and image watermarking \cite{zhu2018hidden}. Section \ref{sec:background} provides the understanding of image watermarking in a graph view, followed by Section \ref{sec:ourconv}, which introduces our convolution on 3D meshes.

\subsection{Background} \label{sec:background}

2D image $F(x,y)$ can be viewed as a weighted graph signal where points are indexed by discrete 2D grid offset $(x,y)\in \mathbb{N}^2$, edges connect, adjacent points and weights are the RGB values of points. Traditional CNN is to apply a filter matrix $W$ of size $(2m+1,2n+1)$ to an image. In this case, the point $(x,y)$ is adjacent to points $(x+\delta x, y+\delta y)$, where $\delta x\in \{-m,...,-1,0,1,...,m\}$, and $\delta y\in\{-n,...,-1,0,1,...,n\}$. Then we can view traditional CNN in a graph way (Eq.(\ref{eq:grapical_cnn})).
\begin{equation}
    \begin{aligned}
        F(x,y) = \sum_{(\delta x, \delta y) \in \mathcal{N}(x,y)}W(\delta x,\delta y)F(x-\delta x,y-\delta y)
    \end{aligned}
    \label{eq:grapical_cnn}
\end{equation}
where $\mathcal{N}(x,y)$ is the set of points adjacent to $(x,y)$, and the filter matrix $W$ can be viewed as a function mapping from grid offsets $(\delta x, \delta y)$ to filter weights. \cite{zhu2018hidden} uses stacked CNN to model both $\mathcal{E}_{\phi}$ and $\mathcal{D}_{\theta}$ (Eq. \ref{eq:problem}). Their method achieves both robust and imperceptible image watermarking. Inspired by their success, we use stacked GAT (Section. \ref{sec:ourconv}) to build our watermark architecture. 

\subsection{Our Approach} \label{sec:ourconv}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/method/distribution_xyz.pdf}
        \caption{Coordinates Distribution}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/method/distribution_relation.pdf}
        \caption{Relation Distribution}
    \end{subfigure}
    \caption{t-SNE \cite{van2008tsne} visualization of the distribution between original and decimated meshes. (a) shows the existence of distribution shifts between the original and decimated coordinates. However, (b) shows that the distributions of decimated relations $D(v_i, v_j)$ are included in the distributions of the original ones.}
    \label{fig:method_distribution_relation_xyz}
\end{figure}

We view 3D mesh $G(V,F)$ as a weighted graph signal where points are indexed by continuous 3D coordinates $(x,y,z)$, edges $E$ can be transformed from faces $F$, and the weights are features $f$ of points.
To watermark a graph signal $G(V, E)$, we naturally consider spectral-based graph convolution \cite{defferrard2016cheby} to perform watermarking tasks. However, spectral-based methods focus on the global feature because they rely on the Laplacian decomposition on the entire graph, which makes them less robust to cropping attacks and less efficient to large graphs. We explore the way of robust embedding by utilizing local features in the spatial domain. We first define our adopted graph attention network as:
\begin{equation}
    \begin{gathered}
        F^{l+1}(v_i)=\frac{1}{|\mathcal{N}(v_i)|}\sum_{v_j\in \mathcal{N}(v_i)}F^l(v_j)W_{\Theta}(D(v_j,v_i))
    \end{gathered}
    \label{eq:3Dconv}
\end{equation}
The feature vector $F^{l+1}(v_i)$ is a weighted sum of the features $F^{l}(v_j)$ in its neighborhoods $v_j\in \mathcal{N}(v_i)$. The neighborhood $\mathcal{N}(v_i)=\{v_j, (v_j, v_i)\in E\}\cup \{v_i\}$ is defined as all points adjacent to the point $v_i$ and itself. The weight $W:\mathbb{R}^3\mapsto \mathbb{R}^d$ is dynamically generated based on the relation $D(v_i, v_j)$ between $v_i$ and $v_j$ and we model $W$ using a parameterized learnable network.

We show that it is beneficial to learn from relation $D(v_i, v_j)$ distributions instead of coordinates distributions. We define $D(v_i, v_j)$ as the coordinate offset from $v_i$ to $v_j$. Figure \ref{fig:method_distribution_relation_xyz} shows that such relations can survive the mesh decimation algorithm because the decimated relation is still included in the original ones (Fig.\ref{fig:method_distribution_relation_xyz} (b)) while coordinates distribution shifts from the original after decimation process (Fig. \ref{fig:method_distribution_relation_xyz} (a)). Based on this insight, our method is trained on simplified meshes.
%TODO extensive experiments
